Jointly Generating Multi-view Consistent PBR Textures using Collaborative Control

Multi-view consistency remains a challenge for image diffusion models. Even within the Text-to-Texture problem, where perfect geometric correspondences are known a priori, many methods fail to yield aligned predictions across views, necessitating non-trivial fusion methods to incorporate the results onto the original mesh. We explore this issue for a Collaborative Control workflow specifically in PBR Text-to-Texture. Collaborative Control directly models PBR image probability distributions, including normal bump maps; to our knowledge, the only diffusion model to directly output full PBR stacks. We discuss the design decisions involved in making this model multi-view consistent, and demonstrate the effectiveness of our approach in ablation studies, as well as practical applications.

==> compile_out <==
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2023-11-01>
L3 programming layer <2023-11-09>
(./llncs.cls
Document Class: llncs 2022/09/05 v2.22 
 LaTeX document class for Lecture Notes in Computer Science
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/article.cls
Document Class: article 2023/05/17 v1.4n Standard LaTeX document class
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/size10.clo))
(/usr/local/texlive/2023/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/oberdiek/aliascnt.sty))
(./eccv.sty (/usr/local/texlive/2023/texmf-dist/tex/latex/silence/silence.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/lineno/lineno.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2023/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics-def/pdftex.def)
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/dvipsnam.def)
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/caption/subcaption.sty))
(./preamble.tex (/usr/local/texlive/2023/texmf-dist/tex/latex/base/fontenc.sty)
 (/usr/local/texlive/2023/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/tools/array.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/fontawesome5/fontawesome5.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))
(/usr/local/texlive/2023/texmf-dist/tex/latex/l3packages/l3keys2e/l3keys2e.sty)
 (/usr/local/texlive/2023/texmf-dist/tex/latex/l3packages/xparse/xparse.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/fontawesome5/fontawesome5-generic
-helper.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/fontawesome5/fontawesome5-mapping
.def))) (/usr/local/texlive/2023/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/overpic/overpic.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/eepic/epic.sty
Enhancements to Picture Environment. Version 1.2 - Released June 1, 1986
)) (/usr/local/texlive/2023/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2023/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2023/texmf-dist/tex/latex/l3packages/xfrac/xfrac.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/l3packages/xtemplate/xtemplate.st
y)) (/usr/local/texlive/2023/texmf-dist/tex/latex/colortbl/colortbl.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/lipsum/lipsum.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/lipsum/lipsum.ltd.tex))
(/usr/local/texlive/2023/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2023/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/arydshln/arydshln.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/axessibility/axessibility.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2023/texmf-dist/tex/latex/accsupp/accsupp.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pdfescape/pdfescape.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/local/texlive/2023/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/accsupp/accsupp-pdftex.def))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pdftex/glyphtounicode.tex))
(/usr/local/texlive/2023/texmf-dist/tex/latex/pdflscape/pdflscape.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/pdflscape/pdflscape-nometadata.st
y (/usr/local/texlive/2023/texmf-dist/tex/latex/graphics/lscape.sty)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/algorithmicx/algpseudocode.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/algorithmicx/algorithmicx.sty
Document Style algorithmicx 1.2 - a greatly improved `algorithmic' style
)
Document Style - pseudocode environments for use with the `algorithmicx' style
) (/usr/local/texlive/2023/texmf-dist/tex/latex/siunitx/siunitx.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/translations/translations.sty))
(/usr/local/texlive/2023/texmf-dist/tex/generic/soul/soul.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/soul/soul-ori.sty)
(/usr/local/texlive/2023/texmf-dist/tex/generic/etexcmds/etexcmds.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.te
x)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgfkeyslibraryfil
tered.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.d
ef
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-p
df.def)))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.
code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.
code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.
tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic
.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigo
nometric.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.rando
m.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.compa
rison.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.
code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round
.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.
code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integ
erarithmetics.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex)
) (/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.co
de.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconst
ruct.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage
.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.co
de.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicst
ate.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransform
ations.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.cod
e.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.c
ode.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathproce
ssing.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.co
de.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.cod
e.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.cod
e.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.
code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.co
de.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretranspare
ncy.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.
code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.
tex)))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.cod
e.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.
tex)
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-0-65.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-1-18.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex)
) (/usr/local/texlive/2023/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex))

(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.cod
e.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothan
dlers.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.cod
e.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarytopaths.code.tex)))
(/usr/local/texlive/2023/texmf-dist/tex/latex/pgfplots/pgfplots.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplots.revision.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplots.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotscore.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/sys/pgfplotssysgeneric
.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/libs/pgfplotslibrary.c
ode.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/oldpgfcompatib/pgfplot
soldpgfsupp_loader.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/pgflibraryfpu.cod
e.tex)
Package pgfplots: loading complementary utilities for your pgf version...

(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/oldpgfcompatib/pgfplot
soldpgfsupp_pgfutil-common-lists.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/util/pgfplotsutil.code
.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
liststructure.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
liststructureext.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
array.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
matrix.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/numtable/pgfplotstable
shared.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/liststructure/pgfplots
deque.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/util/pgfplotsbinary.co
de.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/util/pgfplotsbinary.da
ta.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/util/pgfplotsutil.verb
.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/libs/pgflibrarypgfplot
s.surfshading.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/sys/pgflibrarypgfplots
.surfshading.pgfsys-pdftex.def)))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/util/pgfplotscolormap.
code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/util/pgfplotscolor.cod
e.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotsstackedplots.c
ode.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotsplothandlers.c
ode.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotsmeshplothandle
r.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotsmeshplotimage.
code.tex)))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplots.scaling.code.
tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotscoordprocessin
g.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplots.errorbars.cod
e.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplots.markers.code.
tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplotsticks.code.tex
)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/pgfplots.paths.code.te
x)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/modules/pgfmoduledecoration
s.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathmorphing.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathmorphing.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathreplacing.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathreplacing.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgfplots/libs/tikzlibrarypgfplo
ts.contourlua.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryplotmarks.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/pgflibraryplotmar
ks.code.tex)))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.geometric.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.geometric.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.misc.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.misc.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.symbols.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.symbols.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.arrows.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.arrows.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.callouts.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.callouts.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.multipart.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.multipart.code.tex)))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarycalc.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarybackgrounds.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarypositioning.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryarrows.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/pgflibraryarrows.
code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/pgflibraryarrows.
meta.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.text.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.text.code.tex))
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryfit.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryspy.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrary3d.code.tex)
(/usr/local/texlive/2023/texmf-dist/tex/latex/spath3/tikzlibrarycalligraphy.cod
e.tex (/usr/local/texlive/2023/texmf-dist/tex/latex/spath3/spath3.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/tcolorbox/tcolorbox.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/environ/environ.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/tcolorbox/tcbskins.code.tex
Library (tcolorbox): 'tcbskins.code.tex' version '6.1.0'
(/usr/local/texlive/2023/texmf-dist/tex/latex/tikzfill/tikzfill.image.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/tikzfill/tikzfill-common.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/tikzfill/tikzlibraryfill.image.co
de.tex))
(/usr/local/texlive/2023/texmf-dist/tex/latex/tcolorbox/tcbskinsjigsaw.code.tex
Library (tcolorbox): 'tcbskinsjigsaw.code.tex' version '6.1.0'
))) (/usr/local/texlive/2023/texmf-dist/tex/latex/psnfss/pifont.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/psnfss/upzd.fd)
(/usr/local/texlive/2023/texmf-dist/tex/latex/psnfss/upsy.fd))
(/usr/local/texlive/2023/texmf-dist/tex/latex/blindtext/blindtext.sty)
(./colors.tex)) (./eccvabbrv.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2023/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (/usr/local/texlive/2023/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2023/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2023/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2023/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2023/texmf-dist/tex/latex/orcidlink/orcidlink.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarysvg.path.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/libraries/pgflibrarysvg.pat
h.code.tex
(/usr/local/texlive/2023/texmf-dist/tex/generic/pgf/modules/pgfmoduleparser.cod
e.tex)))) (/usr/local/texlive/2023/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2023/texmf-dist/tex/generic/iftex/ifvtex.sty))
(/usr/local/texlive/2023/texmf-dist/tex/latex/cleveref/cleveref.sty)
(./main.aux (./fig/all_attention.aux) (./fig/multiview_attention.aux)
(./fig/pointwise_attention.aux))
(/usr/local/texlive/2023/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2023/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2023/texmf-dist/tex/latex/grfext/grfext.sty)
(/usr/local/texlive/2023/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2023/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2023/texmf-dist/tex/latex/translations/translations-basic-d
ictionary-english.trsl)
Package pgfplots notification 'compat/show suggested version=true': you might b
enefit from \pgfplotsset{compat=1.18} (current compat level: 1.14).

(./main.out) (./main.out)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2023/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2023/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2023/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(/usr/local/texlive/2023/texmf-dist/tex/latex/base/t1cmtt.fd)
Title too long for running head. Please supply
a shorter form with \titlerunning prior to \maketitle
(./sec/0_abstract.tex) (./sec/1_introduction.tex [1{/usr/local/texlive/2023/tex
mf-var/fonts/map/pdftex/updmap/pdftex.map}{/usr/local/texlive/2023/texmf-dist/f
onts/enc/dvips/cm-super/cm-super-t1.enc}{/usr/local/texlive/2023/texmf-dist/fon
ts/enc/dvips/cm-super/cm-super-ts1.enc} <./fig/teaser/natural_scene.png> <./fig
/teaser/golden_scene.png> <./fig/teaser/steampunk_scene.png> <./fig/teaser/sand
stone_scene.png> <./fig/teaser/naked_scene.png> <./fig/teaser/steampunk_bear.pn
g (PNG copy)>]) (./sec/2_related.tex [2 <./fig/fantasia3d-fig4-albedo.png> <./f
ig/CC-albedo2.png> <./fig/artist-albedo2.png>] [3]) (./sec/3_method.tex

Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 6.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 6.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 11.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 11.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 16.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 16.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 21.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 21.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 26.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 26.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 31.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 31.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 36.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 36.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 41.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 41.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 46.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 46.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyinnode''? on in
put line 51.


Package pgf Warning: Returning node center instead of a point on node border. D
id you specify a point identical to the center of node ``tikzspyonnode''? on in
put line 51.

[4 <./fig/artists_object/albedo1.png> <./fig/artists_object/roughness1.png> <./
fig/artists_object/metallic1.png> <./fig/artists_object/bumps1.png> <./fig/arti
sts_object/render1.png> <./fig/artists_object/albedo2.png> <./fig/artists_objec
t/roughness2.png> <./fig/artists_object/metallic2.png> <./fig/artists_object/bu
mps2.png> <./fig/artists_object/render2.png>] (./fig/all_attention.tex

LaTeX Font Warning: Font shape `T1/cmr/m/n' in size <28> not available
(Font)              size <29.86> substituted on input line 113.


LaTeX Font Warning: Font shape `OT1/cmr/m/n' in size <28> not available
(Font)              size <24.88> substituted on input line 113.


LaTeX Font Warning: Font shape `OT1/cmr/m/n' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.


LaTeX Font Warning: Font shape `OML/cmm/m/it' in size <28> not available
(Font)              size <24.88> substituted on input line 113.


LaTeX Font Warning: Font shape `OML/cmm/m/it' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.


LaTeX Font Warning: Font shape `OMS/cmsy/m/n' in size <28> not available
(Font)              size <24.88> substituted on input line 113.


LaTeX Font Warning: Font shape `OMS/cmsy/m/n' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.


LaTeX Font Warning: Font shape `OT1/cmr/bx/n' in size <28> not available
(Font)              size <24.88> substituted on input line 113.


LaTeX Font Warning: Font shape `OT1/cmr/bx/n' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.


LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <28> not available
(Font)              size <24.88> substituted on input line 113.


LaTeX Font Warning: Font shape `OML/cmm/b/it' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.


LaTeX Font Warning: Font shape `OMS/cmsy/b/n' in size <28> not available
(Font)              size <24.88> substituted on input line 113.


LaTeX Font Warning: Font shape `OMS/cmsy/b/n' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.


LaTeX Font Warning: Font shape `T1/cmr/m/n' in size <19.59991> not available
(Font)              size <20.74> substituted on input line 113.

) (./fig/multiview_attention.tex) [5] (./fig/pointwise_attention.tex

LaTeX Font Warning: Font shape `T1/cmr/m/n' in size <16> not available
(Font)              size <17.28> substituted on input line 126.


(/usr/local/texlive/2023/texmf-dist/tex/latex/fontawesome5/ufontawesomefree1.fd
)) [6] [7{/usr/local/texlive/2023/texmf-dist/fonts/enc/dvips/fontawesome5/fa5fr
ee1.enc}]) (./sec/4_results.tex [8] [9 <./fig/mvdata_example/0001.png> <./fig/m
vdata_example/0002.png> <./fig/mvdata_example/0003.png> <./fig/mvdata_example/0
004.png> <./fig/mvdata_example/0005.png> <./fig/mvdata_example/0006.png> <./fig
/mvdata_example/0007.png> <./fig/mvdata_example/0008.png> <./fig/mvdata_example
/0009.png> <./fig/mvdata_example/0010.png> <./fig/mvdata_example/0011.png> <./f
ig/mvdata_example/0012.png> <./fig/mvdata_example/0013.png> <./fig/mvdata_examp
le/0014.png> <./fig/mvdata_example/0015.png> <./fig/mvdata_example/0016.png>]
(./fig/pixelwise_ablation.tex (./fig/auto_collected/no_pointwise_prompt.txt))

Package caption Warning: The option `hypcap=true' will be ignored for this
(caption)                particular \caption on input line 50.
See the caption package documentation for explanation.

(./fig/occlusion_ablation.tex (./fig/auto_collected/no_occlusions_prompt.txt))

Package caption Warning: The option `hypcap=true' will be ignored for this
(caption)                particular \caption on input line 57.
See the caption package documentation for explanation.

[10 <./fig/auto_collected/no_pointwise_reference.png (PNG copy)> <./fig/auto_co
llected/no_pointwise_baseline_albedo0.png (PNG copy)> <./fig/auto_collected/no_
pointwise_baseline_albedo1.png (PNG copy)> <./fig/auto_collected/no_pointwise_b
aseline_roughness1.png (PNG copy)> <./fig/auto_collected/no_pointwise_baseline_
metallic1.png (PNG copy)> <./fig/auto_collected/no_pointwise_baseline_render.pn
g (PNG copy)> <./fig/auto_collected/no_pointwise_ablated_albedo0.png (PNG copy)
> <./fig/auto_collected/no_pointwise_ablated_albedo1.png (PNG copy)> <./fig/aut
o_collected/no_pointwise_ablated_roughness1.png (PNG copy)> <./fig/auto_collect
ed/no_pointwise_ablated_metallic1.png (PNG copy)> <./fig/auto_collected/no_poin
twise_ablated_render.png (PNG copy)> <./fig/auto_collected/no_occlusions_refere
nce.png (PNG copy)> <./fig/auto_collected/no_occlusions_baseline_roughness0.png
 (PNG copy)> <./fig/auto_collected/no_occlusions_baseline_roughness1.png (PNG c
opy)> <./fig/auto_collected/no_occlusions_baseline_albedo1.png (PNG copy)> <./f
ig/auto_collected/no_occlusions_baseline_metallic1.png (PNG copy)> <./fig/auto_
collected/no_occlusions_baseline_render.png (PNG copy)> <./fig/auto_collected/n
o_occlusions_ablated_roughness0.png (PNG copy)> <./fig/auto_collected/no_occlus
ions_ablated_roughness1.png (PNG copy)> <./fig/auto_collected/no_occlusions_abl
ated_albedo1.png (PNG copy)> <./fig/auto_collected/no_occlusions_ablated_metall
ic1.png (PNG copy)> <./fig/auto_collected/no_occlusions_ablated_render.png (PNG
 copy)>] (./fig/refhid_ablation.tex
(./fig/auto_collected/no_ref_attention_prompt.txt))

Package caption Warning: The option `hypcap=true' will be ignored for this
(caption)                particular \caption on input line 70.
See the caption package documentation for explanation.

(./fig/dino_ablation.tex (./fig/auto_collected/no_dino_prompt.txt))

Package caption Warning: The option `hypcap=true' will be ignored for this
(caption)                particular \caption on input line 77.
See the caption package documentation for explanation.

(./fig/view_scale_ablation.tex (./fig/auto_collected/with_zoomin_prompt.txt)
Overfull \hbox (1.14717pt too wide) in paragraph at lines 53--53
 [][][]\T1/cmr/m/n/5 (-20) Visualization 

Overfull \hbox (1.14717pt too wide) in paragraph at lines 53--53
 [][][]\T1/cmr/m/n/5 (-20) Visualization 

Overfull \hbox (1.14717pt too wide) in paragraph at lines 53--53
 [][][]\T1/cmr/m/n/5 (-20) Visualization 
)
Underfull \vbox (badness 1406) has occurred while \output is active [11 <./fig/
auto_collected/no_ref_attention_reference.png (PNG copy)> <./fig/auto_collected
/no_ref_attention_baseline_albedo0.png (PNG copy)> <./fig/auto_collected/no_ref
_attention_baseline_albedo1.png (PNG copy)> <./fig/auto_collected/no_ref_attent
ion_baseline_roughness1.png (PNG copy)> <./fig/auto_collected/no_ref_attention_
baseline_metallic1.png (PNG copy)> <./fig/auto_collected/no_ref_attention_basel
ine_render.png (PNG copy)> <./fig/auto_collected/no_ref_attention_ablated_albed
o0.png (PNG copy)> <./fig/auto_collected/no_ref_attention_ablated_albedo1.png (
PNG copy)> <./fig/auto_collected/no_ref_attention_ablated_roughness1.png (PNG c
opy)> <./fig/auto_collected/no_ref_attention_ablated_metallic1.png (PNG copy)> 
<./fig/auto_collected/no_ref_attention_ablated_render.png (PNG copy)> <./fig/au
to_collected/no_dino_reference.png (PNG copy)> <./fig/auto_collected/no_dino_ba
seline_albedo0.png (PNG copy)> <./fig/auto_collected/no_dino_baseline_albedo1.p
ng (PNG copy)> <./fig/auto_collected/no_dino_baseline_roughness1.png (PNG copy)
> <./fig/auto_collected/no_dino_baseline_metallic1.png (PNG copy)> <./fig/auto_
collected/no_dino_baseline_render.png (PNG copy)> <./fig/auto_collected/no_dino
_ablated_albedo0.png (PNG copy)> <./fig/auto_collected/no_dino_ablated_albedo1.
png (PNG copy)> <./fig/auto_collected/no_dino_ablated_roughness1.png (PNG copy)
> <./fig/auto_collected/no_dino_ablated_metallic1.png (PNG copy)> <./fig/auto_c
ollected/no_dino_ablated_render.png (PNG copy)>] (./fig/superres_demo.tex
Overfull \hbox (1.14717pt too wide) in paragraph at lines 53--53
 [][][]\T1/cmr/m/n/5 (-20) Visualization 

Overfull \hbox (1.14717pt too wide) in paragraph at lines 53--53
 [][][]\T1/cmr/m/n/5 (-20) Visualization 

Overfull \hbox (1.14717pt too wide) in paragraph at lines 53--53
 [][][]\T1/cmr/m/n/5 (-20) Visualization 
) [12 <./fig/auto_collected/with_zoomin_reference.png (PNG copy)> <./fig/auto_c
ollected/with_zoomin_baseline_albedo4.png (PNG copy)> <./fig/auto_collected/wit
h_zoomin_baseline_albedo2.png (PNG copy)> <./fig/auto_collected/with_zoomin_bas
eline_albedo3.png (PNG copy)> <./fig/auto_collected/with_zoomin_baseline_albedo
1.png (PNG copy)> <./fig/auto_collected/with_zoomin_ablated_albedo4.png (PNG co
py)> <./fig/auto_collected/with_zoomin_ablated_albedo2.png (PNG copy)> <./fig/a
uto_collected/with_zoomin_ablated_albedo3.png (PNG copy)> <./fig/auto_collected
/with_zoomin_ablated_albedo1.png (PNG copy)> <./fig/auto_collected/with_zoomin_
ablated_albedo5.png (PNG copy)> <./fig/auto_collected/superres1_albedo0.png (PN
G copy)> <./fig/auto_collected/superres1_albedo1.png (PNG copy)> <./fig/auto_co
llected/superres2_albedo0.png (PNG copy)> <./fig/auto_collected/superres2_albed
o1.png (PNG copy)> <./fig/auto_collected/superres3_albedo0.png (PNG copy)> <./f
ig/auto_collected/superres3_albedo1.png (PNG copy)>]
(./fig/bump_map_ablation.tex (./fig/auto_collected/no_bumps_prompt.txt)
(./fig/auto_collected/no_bumps2_prompt.txt))) (./sec/5_conclusion.tex [13 <./fi
g/auto_collected/vs_flashtex_flashtex1_0.png (PNG copy)> <./fig/auto_collected/
vs_flashtex_flashtex1_1.png (PNG copy)> <./fig/auto_collected/vs_flashtex_flash
tex2_0.png (PNG copy)> <./fig/auto_collected/vs_flashtex_flashtex2_1.png (PNG c
opy)> <./fig/auto_collected/meta_bunnies.png> <./fig/auto_collected/our_bunnies
_softsky.png> <./fig/auto_collected/metatexturegen_armadillo.png> <./fig/auto_c
ollected/metatexturegen_van.png> <./fig/auto_collected/metatexturegen_butterfly
.png> <./fig/auto_collected/our_armadillo.png> <./fig/auto_collected/our_van.pn
g> <./fig/auto_collected/our_butterfly.png> <./fig/auto_collected/vs_flashtex_u
s1_0.png> <./fig/auto_collected/vs_flashtex_us1_1.png> <./fig/auto_collected/vs
_flashtex_us2_0.png> <./fig/auto_collected/vs_flashtex_us2_1.png>]) (./main.bbl

Underfull \vbox (badness 2111) has occurred while \output is active [14 <./fig/
auto_collected/no_bumps_reference.png (PNG copy)> <./fig/auto_collected/no_bump
s_baseline_albedo0.png (PNG copy)> <./fig/auto_collected/no_bumps_baseline_roug
hness0.png (PNG copy)> <./fig/auto_collected/no_bumps_baseline_metallic0.png (P
NG copy)> <./fig/auto_collected/no_bumps_baseline_bumps0.png (PNG copy)> <./fig
/auto_collected/no_bumps_ablated_render.png (PNG copy)> <./fig/auto_collected/n
o_bumps_baseline_render.png (PNG copy)> <./fig/auto_collected/no_bumps2_referen
ce.png (PNG copy)> <./fig/auto_collected/no_bumps2_baseline_albedo0.png (PNG co
py)> <./fig/auto_collected/no_bumps2_baseline_roughness0.png (PNG copy)> <./fig
/auto_collected/no_bumps2_baseline_metallic0.png (PNG copy)> <./fig/auto_collec
ted/no_bumps2_baseline_bumps0.png (PNG copy)> <./fig/auto_collected/no_bumps2_a
blated_render.png (PNG copy)> <./fig/auto_collected/no_bumps2_baseline_render.p
ng (PNG copy)>] [15] [16] [17]
Underfull \hbox (badness 6284) in paragraph at lines 305--308
[]\T1/cmr/m/n/9 (+20) Teczan, K.: Free game char-ac-ter - an-cient sketch-fab m
odel, []$\T1/cmtt/m/n/9 https :

Underfull \hbox (badness 10000) in paragraph at lines 305--308
\T1/cmtt/m/n/9 / / sketchfab . com / 3d -[] models / free -[] game -[] characte
r -[] ancient -[]

Underfull \hbox (badness 1275) in paragraph at lines 326--329
[]\T1/cmr/m/n/9 (+20) Wang, Z., Xu, Q., Tan, F., Chai, M., Liu, S., Pandey, R.,
 Fanello, S.,
[18]) [19] (./main.aux (./fig/all_attention.aux) (./fig/multiview_attention.aux
) (./fig/pointwise_attention.aux))

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 3.12pt have occurred.

 )
(see the transcript file for additional information)</usr/local/texlive/2023/te
xmf-dist/fonts/type1/public/fontawesome5/FontAwesome5Free-Solid.pfb></usr/local
/texlive/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx9.pfb></usr/local/t
exlive/2023/texmf-dist/fonts/type1/public/amsfonts/cmextra/cmex9.pfb></usr/loca
l/texlive/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local
/texlive/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></usr/local/
texlive/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/te
xlive/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texl
ive/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texliv
e/2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi9.pfb></usr/local/texlive/
2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmmib10.pfb></usr/local/texlive/
2023/texmf-dist/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/20
23/texmf-dist/fonts/type1/public/amsfonts/cm/cmr17.pfb></usr/local/texlive/2023
/texmf-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2023/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/local/texlive/2023/texmf
-dist/fonts/type1/public/amsfonts/cm/cmr9.pfb></usr/local/texlive/2023/texmf-di
st/fonts/type1/public/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2023/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmsy6.pfb></usr/local/texlive/2023/texmf-dist/
fonts/type1/public/amsfonts/cm/cmsy7.pfb></usr/local/texlive/2023/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmsy9.pfb></usr/local/texlive/2023/texmf-dist/font
s/type1/public/cm-super/sfbx0700.pfb></usr/local/texlive/2023/texmf-dist/fonts/
type1/public/cm-super/sfbx0900.pfb></usr/local/texlive/2023/texmf-dist/fonts/ty
pe1/public/cm-super/sfbx1000.pfb></usr/local/texlive/2023/texmf-dist/fonts/type
1/public/cm-super/sfbx1200.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/
public/cm-super/sfbx1440.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/pu
blic/cm-super/sfrm0500.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/publ
ic/cm-super/sfrm0700.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public
/cm-super/sfrm0900.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/c
m-super/sfrm1000.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-
super/sfrm1728.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-su
per/sfrm2074.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-supe
r/sfrm2986.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-super/
sfti0900.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-super/sf
ti1000.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-super/sftt
0900.pfb></usr/local/texlive/2023/texmf-dist/fonts/type1/public/cm-super/sftt10
00.pfb>
Output written on main.pdf (19 pages, 86328730 bytes).
Transcript written on main.log.

